Modular Networks for Validating Community Detection Algorithms

How can we accurately compare different community detection algorithms? These algorithms cluster nodes in a given network, and their performance is often validated on benchmark networks with explicit ground-truth communities. Given the lack of cluster labels in real-world networks, a model that generates realistic networks is required for accurate evaluation of these algorithm. In this paper, we present a simple, intuitive, and flexible benchmark generator to generate intrinsically modular networks for community validation. We show how the generated networks closely comply with the characteristics observed for real networks; whereas their characteristics could be directly controlled to match wide range of real world networks. We further show how common community detection algorithms rank differently when being evaluated on these benchmarks compared to current available alternatives.

==> 8_algos.tex <==
 
 
\newcommand{\nl}{\STATE}
\newcommand{\nlx}{\STATEx}
\newcommand{\BlankLine}{}
% \newcommand{\ForEach}{\For}
\newcommand{\tcc}{ \COMMENT}
\newcommand{\ForEach}[2]{\FOR{#1}#2\ENDFOR}
% \newcommand{\For}[2]{\FOR{#1}#2\ENDFOR}
\newcommand{\While}[2]{\WHILE{#1}#2\ENDWHILE}
\newcommand{\If}[2]{\IF{#1}#2\ENDIF}
\newcommand{\lIf}[2]{\STATE \textbf{if} #1 \textbf{then} #2}
\newcommand{\lFor}[2]{\STATE \textbf{for}\ {#1}\textbf{ do}#2}
\newcommand{\lEIf}[3]{\IF{#1} #2 \ELSE #3 \ENDIF}
\newcommand{\lElse}[2]{\STATE \textbf{else} #1}
\newcommand{\DontPrintSemicolon}{}
\newcommand{\tcp}[1]{\COMMENT{#1}}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \algsetup{linenodelimiter=.}
\newcommand{\Rep}[2]{\REPEAT { #1} \textbf{times} #2 \UNTIL{}}
\renewcommand{\algorithmicuntil}{\textbf{end repeat}}
% \newcommand{\KwIn}[1]{\REQUIRE #1}
% \newcommand{\KwOut}[1]{\ENSURE #1}
 
 % This can be summarized as:
% \begin{enumerate}
% \item{\textsl{realize}:}
% $G \leftarrow \mathcal{M}(\theta^{G}) $
% \item{\textsl{assign}:}
% $C \leftarrow assign(G, \theta^{C}) $
% \item{\textsl{overlay}:}
% $G, C \leftarrow overlay(G,C, \theta^{C}) $
% \end{enumerate}
 % summarized in \refalg{alg:twopass}. 

%  The LFR benchmarks use CF as the 
% i, asa two-pass benchmark generator;  as summarized in . 
%  It first, generates a network, and then overlays a community structure on this network.
% \newcommand{\ctcc}[1]{{\small\color{OliveGreen}\tcc{#1}}}
% \newcommand{\ctcp}[1]{{\small\color{OliveGreen}\tcp*[r]{#1}}}
%\vspace{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}
% % \SetKwInOut{Parameters}{params}
% \SetKwInOut{Output}{output}
% %\Fn {Assign}
% { 
% \Input{Network model $\mathcal{M}$, parameters of network $\theta^{G}$, and parameters of communities $\theta^{C}$} 
% % \Parameters{network prameters $\theta$}
% % \Parameters{for communities}
% \Output{A randomly generated benchmark} 
% \BlankLine
% % \nlset{P1}\Begin{ 
% \ctcc{realize a network}
% \nl $G \leftarrow \mathcal{M}(\theta^{G}) $\;
% \ctcc{assign nodes to communities}
% \nl $C \leftarrow assign(G, \theta^{C}) $\;
% % \ctcc{determine number of communities}
% % \nl determine $m$ based on $\theta^{C}_m$ \;
% % \ctcc{initialize the communities}
% % \nl$C \leftarrow \{c_1=\emptyset, c_2 =\emptyset \ldots c_m =\emptyset \} $\;
% % \ctcc{determine capacity of communities}
% % \nl$N \leftarrow \{ (1,n_1), (2,n_2) \ldots (m,n_{m}) \}$ based on $\theta^{C}$\;
% % }
% % \nlset{P2}\Begin{ 
% % \nl\For{$v$ in $G$}{
% % \nl\For{$c$ in $assignments(v)$}{
% % }
% % \nl$i \leftarrow rand(1, |N|)$ \;
% % \nl$C_{N_{i}.{first}} \leftarrow v$ \;
% % \nl$N_{i}.{second} \leftarrow N_{i}.{second}-1$ \;
% % \nl\lIf{$N_{i}.{second}=0$ }{ remove $N_{i}$ form $N$ }
% % }
% %\ctcc{rewire edges}
% % \While {not satisfied$(G,C, \theta^{C})$}{
% % $G, C \leftarrow adjust(G,C, \theta^{C}) $\;
% % }
% \ctcc{overlay communities}
% \nl $G, C \leftarrow overlay(G,C, \theta^{C}) $\;
% \BlankLine
% % }
%  \Return $G,C$}
% \caption{Three Pass Benchmark Generator.%. Network model $\mathcal{M}$, parameters of network $\theta_{N}$, and parameters of communities $\theta_{C}$
% }
% \label{alg:twopass}
% \end{algorithm} 
% \subsection{Generalized Three-Pass Benchmark Generator}
% \label{ap:twopass}
%  The generalized three-pass benchmark generator for community mining algorithms is summarized in 
%  \refalg{alg:twopass}; which simply first, generates a network according to the given parameters $\theta^{G}$, second, creates a communities based on the given parameters, $\theta^{C}$ and assign the nodes to these communities, and third, overlays this community structure on the network, to satisfy the constraints given in $\theta^{C}$.
% % \newcommand{\ctcc}[1]{{\small\color{OliveGreen}\tcc{#1}}}
% % \newcommand{\ctcp}[1]{{\small\color{OliveGreen}\tcp*[r]{#1}}}
% 
% %\vspace{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}
% % \SetKwInOut{Parameters}{params}
% \SetKwInOut{Output}{output}
% %\Fn {Assign}
% { 
% \Input{Network model $\mathcal{M}$, parameters of network $\theta^{G}$, and parameters of communities $\theta^{C}$} 
% % \Parameters{network prameters $\theta$}
% % \Parameters{for communities}
% \Output{A randomly generated benchmark} 
% \BlankLine
% % \nlset{P1}\Begin{ 
% \ctcc{realize a network}
% \nl $G \leftarrow \mathcal{M}(\theta^{G}) $\;
% \ctcc{assign nodes to communities}
% \nl $C \leftarrow assign(G, \theta^{C}) $\;
% % \ctcc{determine number of communities}
% % \nl determine $m$ based on $\theta^{C}_m$ \;
% % \ctcc{initialize the communities}
% % \nl$C \leftarrow \{c_1=\emptyset, c_2 =\emptyset \ldots c_m =\emptyset \} $\;
% % \ctcc{determine capacity of communities}
% % \nl$N \leftarrow \{ (1,n_1), (2,n_2) \ldots (m,n_{m}) \}$ based on $\theta^{C}$\;
% % }
% % \nlset{P2}\Begin{ 
% % \nl\For{$v$ in $G$}{
% % \nl\For{$c$ in $assignments(v)$}{
% % }
% % \nl$i \leftarrow rand(1, |N|)$ \;
% % \nl$C_{N_{i}.{first}} \leftarrow v$ \;
% % \nl$N_{i}.{second} \leftarrow N_{i}.{second}-1$ \;
% % \nl\lIf{$N_{i}.{second}=0$ }{ remove $N_{i}$ form $N$ }
% % }
% %\ctcc{rewire edges}
% % \While {not satisfied$(G,C, \theta^{C})$}{
% % $G, C \leftarrow adjust(G,C, \theta^{C}) $\;
% % }
% \ctcc{overlay communities}
% \nl $G, C \leftarrow overlay(G,C, \theta^{C}) $\;
% \BlankLine
% % }
%  \Return $G,C$}
% \caption{Three Pass Benchmark Generator.%. Network model $\mathcal{M}$, parameters of network $\theta_{N}$, and parameters of communities $\theta_{C}$
% }
% \label{alg:twopass}
% \end{algorithm} 
%\section{Algorithms}
\section{Generalized 3-Pass Benchmark}
%
\subsection{Phase 2: Assign}
\refalg{alg:lfrAssign} summarizes %\footnote{The exact procedure is more complicated and includes ``kicking out'' randomly selected nodes form communities, in order to assign all homeless nodes to communities with size greater than their internal G.degree.} 
the assignment of nodes to communities, which has two main phases, \\
\emph{1) Determine the community sizes:}
By sampling from the community size distribution. Sample communities until the sum of all community sizes equals the total number of nodes. \\%This is the same as LFR.
\emph{2) Assign nodes to the communities:}
First select a random node in the network and add it, %and all of its neighbours, into the same community (
if its degree is less than the size of the community. %This way we limit the amount of re-wiring we need to do since these nodes are already connected. Continue this neighbourhood expansion until the community is full, then restart on a new community. 
Any vertex that is too big for the current community gets put aside.
%
At the end of the community assignment, any nodes that left over are randomly added to a community that is big enough to contain their degree. If that community is already full, then it ejects a smaller-degree node and adds in the left over node. The ejected node then gets added into the leftover node queue. The process continues until there is no left over nodes.

\begin{algorithm}
\vspace{10pt}
\caption{Assign($G$, $\theta^{C}$)}%. Network model $\mathcal{M}$, parameters of network $\theta_{N}$, and parameters of communities $\theta_{C}$
\label{alg:lfrAssign}
\begin{algorithmic}[1]
% \KwIn{Input}{input}
% \SetKwInOut{Output}{output}
% \Input{Network $G$, and parameters of communities $\theta^{C}$} 
% \Output{Resulted communities} 
\BlankLine
% \ctcc{determine number of communities}
% \nl determine $m$ based on $\theta^{C}_m$ \;
\nl $\{s_1, s_2 \ldots s_{m} \}$ based on $\theta^{C}$ and $G$
\ctcc{determine capacity of communities}
\nl $\{c_1=\emptyset, c_2 =\emptyset \ldots c_m =\emptyset \} $% \underbrace{\emptyset, \ldots ,\emptyset}_{m} \}$\;
\ctcc{initialize the communities}
% $N \overset{\quad\theta^{C}}{\Leftarrow} \{ <1,n_1>, <2,n_2> \ldots <m,n_{m}> \}$\;
% \ctcc{put all nodes in homeless queue}
\nl $H \leftarrow \emptyset$
\ctcc{initialize the homeless queue}
\ForEach{$v \in G$}{
\ctcc{assign nodes to communities}
\nl randomly choose $c_i$ from $C$ where $s_i>|c_i|$ 
% \ctcc{pick a community at random}
\lEIf{$s_{i}\geq (1-\mu) \times G.degree(v)$}{$c_{i} .add(v)$ } %\ctcc{assign to  community if fits}
{ $\;H.add(v)$}
%  \ctcc{add to the homeless queue}
% \lElse
}
\While{$H$ is not empty}{
\ctcc{assign homeless nodes }
\nl randomly choose $v$ from $H$\;
\nl$i \leftarrow rand(1, m)$ \;
\ctcc{pick a community at random}
% \ctcc{if internal G.degree is smaller than the community size}
\If{$s_{i}\geq  (1-\mu) \times G.degree(v)$}{
\nl$c_{i} .add(v)$ \;
\nl $H.remove(v)$\;
 \If {$|c_{i}| > s_i$ }{
\ctcc{kick out a random node}
\nl randomly choose $u$ form $c_{i}$\;
\nl $c_i.remove(u)$\;% \leftarrow c_m-u$\;
\nl $H.add(u)$\;
}
}
}
% \Return $\{c_1, c_2,\ldots, c_m \} $
\end{algorithmic}
\end{algorithm} 
\subsubsection{CN Modification}
For the CN assignment, line 5 of the \refalg{alg:lfrAssign} is changed so that the community $c_i$ is chosen from $C$, for node $v$, with probabilities proportional to the current neighbours of $v$ in $c_i$; see \refalg{alg:cnAssign} for the details.  

 \begin{algorithm}\vspace{10pt}
 \caption{CN Assign}
 \label{alg:cnAssign}
\begin{algorithmic}[1]
\addtocounter{ALG@line}{3}
\STATE  $\dots$
\STATE $P  \leftarrow 1 \;\forall c_i \in C$
\addtocounter{ALG@line}{-1}
\FOR{$i \in G.neigh(v)$}\addtocounter{ALG@line}{-1}
\STATE $p_{c_i} \leftarrow p_{c_i}+1$\addtocounter{ALG@line}{-1}
\ENDFOR
\STATE $P \leftarrow P/sum(P)$\addtocounter{ALG@line}{-1}
\STATE  randomly choose $c_i$ from $C$ where $s_i>|c_i|$, and probabilities are proportional to $P$
% \addtocounter{ALG@line}{-1}
\STATE  $\dots$
\end{algorithmic}
 \end{algorithm}


\subsubsection{NE Modification}
For NE assignment, we change line 6-7 of the \refalg{alg:lfrAssign} so that after community $c_i$ is chosen for node $v$, we expand from node $v$ using a BFS(Breadth-first search), to also add its neighbours to $c_i$, until $c_i$ is full or the expansion is ended; see \refalg{alg:neAssign} for details. 

Note that this way of assigning nodes to communities results in far fewer re-wirings because all of the internal edges are already there. Fewer re-wirings yields more realistic network structure.

     
 \begin{algorithm}%[h!]
 \vspace{10pt}
  \caption{NE Assign}
  \label{alg:neAssign}
\begin{algorithmic}[1]
\addtocounter{ALG@line}{4}
\STATE  $\dots$
\STATE $M \leftarrow [0]\times G.n $%\addtocounter{ALG@line}{-1}
\STATE $Q  \leftarrow v$\addtocounter{ALG@line}{-1}
\STATE $M_v \leftarrow 1$\addtocounter{ALG@line}{-1}
\WHILE{$len(Q)>0$ and $c_i<s_i$}\addtocounter{ALG@line}{-1}
	\STATE $v \leftarrow Q.pop$\addtocounter{ALG@line}{-1}
	\STATE $c_i.add(v)$\addtocounter{ALG@line}{-1}
	\IF{$s_i \geq (1-\mu)\times G.degree(v)$}\addtocounter{ALG@line}{-1}
		\STATE $Q.add(v)$\addtocounter{ALG@line}{-1}
		\FOR{$u \in G.neigh(v)$}\addtocounter{ALG@line}{-1}
			\IF{$M_u==0$}\addtocounter{ALG@line}{-1}
				\STATE $Q.add(u)$\addtocounter{ALG@line}{-1}
				\STATE $M_u \leftarrow 1$
			\ENDIF
		\ENDFOR
	\ENDIF
\ENDWHILE
\STATE $\dots$
\end{algorithmic}
 \end{algorithm}

%\newpage
\subsection{Phase 3: Overlay-Rewire}
\refalg{alg:lfrOverlay} summarizes overlay of communities on the network through rewirings. This procedure is not described in details in the authors' original paper \cite{Lancichinetti08LFR}, and the available code for it reflects the modified LFR version\cite{Lancichinetti08overlap}; hence the procedure presented here, is our best guess of the original method.

% 
\emph{1) Determine rewirings:} Each vertex should have $\mu$\% edges leading out of the community (between), and $(1-\mu)$\% edges leading to other nodes in the community (within). So we start by computing how many edges need to rewired for each vertex. For example, Vertex $v$ might need $2$ external edges swapped to internal edges; thus has a desired internal change of $\delta^w=+2$, and a desired external change of $\delta^b=-2$.

\emph{2) Rewire edges within communities: }After computing all the desired changes, iterate through all of the vertices. For each vertex, while it requires more internal edges (i.e. internal change $> 0$ ), we loop through all other vertices that require more internal edges. If there is another vertex in the same community and it requires more internal edges, then we pair them up and add an edge between them (i.e. internal change decreases by one for both). Moreover, we remove the excess internal edges, with a similar process; see line 14-21 of procedure \ref{alg:lfrOverlay} for more details.  %Any vertex that can't reach internal change of zero, is left to be dealt with later.

\emph{3) Rewire edges between communities: }The same process occurs for external change.
In this case we look for other vertices that need an external edge and are out not in the current community of the target vertex. We add an external edge between these two vertices.
% \subsubsection{Final rewirings}
% After all of the internal and external changes are complete, we need to fix the vertices that could not reach their desired within/between edge ratio. This is because there were no open vertices to connect (or sever) ties with. To fix any excess remaining external change requirements, we look through the neighbours of that vertex and simply remove an external edge at random. This means that we will not have the same number of edges as the original network, unfortunately there is no easy way to avoid this. We do the same for vertices that need more external edges (we add an edge at random).  In practice, very few vertices need to be `fixed' so there isn't much adding/removal of edges.
% \newcommand{\tcc}{\}
\begin{algorithm}[t!]%\vspace{10pt}
\caption{Overlay($G$, $C$, $\theta^{C}$)}%. Network model $\mathcal{M}$, parameters of network $\theta_{N}$, and parameters of communities $\theta_{C}$
\label{alg:lfrOverlay}
\begin{algorithmic}[1]
% \KwIn{Input}{input}
% \SetKwInOut{Parameters}{params}
% \SetKwInOut{Output}{output}
% \Input{Network $G$, Communities $C$, and parameters $\theta^{C}$} 
% \Output{Adjusted Network and communities} 
% \BlankLine
\nl $\mu \leftarrow \theta^{C}$\;
\ForEach{$v \in G$}{
\ctcc{determine rewirings per node}
	\nl$ \delta^{b}[v] \leftarrow \lfloor \mu \times deg(v) - deg^b(v,c)\rfloor$ \;
% 	\ctcc{determine desired between changes}
	\nl$ \delta^{w}[v] \leftarrow -\delta^{b}[v] $ \;
	\ctcc{desired within changes}
}
\ForEach{$c \in C$}{
\ctcc{rewire edges within communities}
	\nl $I\leftarrow \{v  \,|\; v\in c \land \delta^{w}[v]> 0 \}$  \;
	\ctcc{add internal edges}
	\While {$|I|\geq  2$}{
		\nl randomly choose $v\neq u$ from $I $\;
		\nl add $edge(u,v)$ to $G$\;
		\nl $\delta^{w}[v] \leftarrow \delta^{w}[v] -1$\;
		\nl $\delta^{w}[u] \leftarrow \delta^{w}[u] -1$\;
		\lIf {$\delta^{w}[v]=0$}{$I.remove(v)$ }
		\lIf {$\delta^{w}[u]= 0$}{$I.remove(u)$ }
	}
	\ForEach {$\{v  \,|\; v\in c \land \delta^{w}[v]< 0 \}$}{
	\ctcc{remove excess edges}
		\nl $I\leftarrow \{u  \,|\; edge(u,v)\in G \land u\in c \land \delta^{w}[u]< 0 \}$  \;
		\While{$|I|\geq 1 \land \delta^{w}[v] <0$}{
			\nl randomly choose $u$ from $I$\;
			\nl remove $edge(u,v)$ from $G$\;
			\nl $\delta^{w}[v] \leftarrow \delta^{w}[v] +1$\;
			\nl $\delta^{w}[u] \leftarrow \delta^{w}[u] +1$\;
% 			\nl \lIf {$\delta^{w}[u]= 0$}{$I.remove(u)$ }
			\nl $I.remove(u)$ 
		}
	}
}
\ForEach{$c \in C$}{
\ctcc{rewire edges between communities }
	\nl $I \leftarrow \{v  \,|\; v\in c \land \delta^{b}[v]> 0 \}$  \;
	\ctcc{add between edges}
	\nl $O \leftarrow \{v  \,|\; v\notin c \land \delta^{b}[v]> 0 \}$  \;	
	\While {$|I|\geq 1 \land |O|\geq 1 $}{
		\nl randomly choose $v$ from $I$\;
		\nl randomly choose $u$ from $O$\;
		\nl add $edge(u,v)$ to $G$\;
		\nl $\delta^{b}[v] \leftarrow \delta^{b}[v] -1$\;
		\nl $\delta^{b}[u] \leftarrow \delta^{b}[u] -1$\;
		 \lIf {$\delta^{b}[v]=0$}{$I.remove(v)$}
		 \lIf {$\delta^{b}[u]=0$}{$O.remove(u)$ }
	}
	\ForEach {$\{v  \,|\; v\in c \land \delta^{b}[v]< 0 \}$}{
	\ctcc{remove excess edges}
		\nl $O\leftarrow \{u  \,|\; edge(u,v)\in G \land u\notin c \land \delta^{b}[u]< 0 \}$  \;
		 \While{$|O|\geq 1 \land \delta^{b}[v] <0$}{
			\nl randomly choose $u$ from $O$\;
			\nl remove $edge(u,v)$ from $G$\;
			\nl $\delta^{b}[v] \leftarrow \delta^{b}[v] +1$\;
			\nl $\delta^{b}[u] \leftarrow \delta^{b}[u] +1$\;
% 			\nl \lIf {$\delta^{b}[u]= 0$}{$O.remove(u)$ }
			\nl $O.remove(u)$ 

		}
	}
}
% \ctcc{final rewirings }
% \nl \Return G,C
% \BlankLine
\end{algorithmic}
\end{algorithm} 

% 
% 1-N		number of nodes
% 1-k		average G.degree
% 1-maxk		maximum G.degree
% 2-mu		mixing parameter
% 1-t1		minus exponent for the G.degree sequence
% 2-t2		minus exponent for the community size distribution
% 2-minc		minimum for the community sizes
% 2-maxc		maximum for the community sizes
% -on		number of overlapping nodes
% -om		number of memberships of the overlapping nodes
% -C              [average clustering coefficient]
\subsection{LFR Generator}
Here we describe LFR in terms of this generalization. %,  then we present the improvements. 
The network model used in the LFR benchmark is the CF model,  described in details in the related work section. 
More specifically, for the LFR, $\theta^G= \{N, k_{avg}, k_{max}, \gamma\}$, which are respectively:  number of nodes in the graph, average G.degree, maximum G.degree and  exponent of power law G.degree distribution. These parameters are basically used to determine the G.degree sequence of $G$; from which the graph is then synthesized using the CF model. 

On the other hand, the parameters for communities are $\theta^C= \{\mu, \beta, c_{min}, c_{max} \}$, which are respectively: mixing parameter, exponent of power law distribution for community sizes, minimum size and maximum size for communities.
The latter three are used to determine the capacity of communities; %, also sampling form a  
whereas the mixing parameter $\mu$ controls the difficulty of problem, which is used in the rewiring phase.

Key issues of LFR benchmarks are discussed in the paper. 
From a technical point of view, the implementation of these benchmarks is heuristic and complex, which rules out modifications as well as analytical analysis. 
When in fact this sampling process of structured networks, does not need to be complicated. An example of unnecessary effort in the original LFR implementation  is many rewirings in order to strictly stick to the exact degree distribution of the nodes, when this degree distribution is itself generated/sampled randomly in the first place. In our implementation of the LFR, we relaxed these restrictions to reach a simpler approach, which is as effective as the original one if not better, since it reduces the amount of rewirings. 

% 
% \section{Justin}
% Here we propose a modified ForestFire model for community benchmark generation. We use this model because the networks it generates satisfy all of the properties of Social Network, including shrinking diameter \cite{Leskovec05ForestFire}.
% % Also it accurately models a real-life twitter network \cite{}. 
% Our modifications are focused on the Ambassador selection stage; more specifically, we select ambassadors with a Preferential Attachment-like algorithm. The probability of choosing an ambassador is not uniform (as in the original FF), but is instead dependent on the G.degree of the node. %See the attached paper for more information.
%We've also attached the modified ForestFire code within the SNAP project. See line 306 in ff.cpp (SNAP->snap->ff.cpp) for the specific code modification that I made. I also enabled the beta parameter in the command line.
% Step 2:
% Import the generated network into JUNG or Meerkat. Simply save the FF network in pairs format, and load it into Meerkat. I have code that already does this, but it's very messy, probably better that you write your own. I've attached my current code (or parts of it at least).
% Step 3:
% After generating the network using the modified ForestFire, we re-wire the network according to the Lancichinetti parameters (mu and community size distribution). In the original Lancichinetti algorithm, it forces all nodes to have an even G.degree. This makes the re-wiring easier, but completely destroys the network properties. Instead we want to preserve the G.degree of each node by using clever re-wiring.
\vspace{10pt}
\section{FARZ}
The procedures for FARZ generator is described in the main paper. The assign algorithm is left out due to its triviality which is described here.
\subsection{FARZ Assign} 
\begin{algorithm}[h!]
\vspace{3pt}
 \caption{FARZ Assign (i, C)}
 \label{alg:farzMain}
\begin{algorithmic}[1]
\FOR{$[ 1\dots r]$}
\STATE $cid \leftarrow select(\{1\dots k\}, p_u = \frac{|u|+\phi}{\sum\limits_{v} (|v|+\phi)})$
\IF{$i\notin C[cid]$} $C[cid] \leftarrow i$ \ENDIF
\ENDFOR
\end{algorithmic}
 \end{algorithm}


==> results_all.tex <==
%\vspace{15pt}
\newpage
\section{Extended Results}
Here we report extended results for the experiments  in the original paper, i.e. distribution plots for all the properties of networks generated by the generalized 3-pass benchmark (in Section \ref{3passres}), and rankings of algorithms in a wider set of settings for the FARZ  (in Section \ref{farzres}). 
%\subsection{Real Networks}
%\begin{figure}[h!]
%\includegraphics[width=.99\linewidth]{figs/realDistnets}
%\caption{Properties of a random \textsl{\citet{Erdos60}} graph, a real-world biological network, and a real-world social network. 
%Real-world networks are known to have a small diameter (small-world), power law degree distribution (scale-free), relatively high transitivity (clustering coefficient), and degree correlation between connecting nodes ((dis-)assortative mixing). } 
%\label{fig:propnets}
%\end{figure}

%\newpage
\subsection{Generalized 3-Pass Benchmark}
\label{3passres}
Complete plots for the properties of the synthesized networks from the different variations derived form our generalized 3-pass model, described in the paper. 
The probability density estimation for parameters, as they change by $\mu$.  In each plot, rows are different models: CF(top), BA(middle), FF(last). Initial network is marked by blue. This corresponds to Figure 3 in the paper. 
 \begin{figure}[h!]
\caption{Original LFR Assignment}
\includegraphics[width=.99\linewidth]{figs/propmuLFR}
\end{figure}
\begin{figure}[h!]
\caption{CN Assignment}
\includegraphics[width=.99\linewidth]{figs/propmuCN}
\end{figure}
\begin{figure}[h!]
\caption{NE Assignment}
\includegraphics[width=.99\linewidth]{figs/propmuNE}
\end{figure}

% \begin{figure*}
% \centering
%  \begin{subfigure}[b]{0.9\textwidth}
%     \includegraphics[width=\textwidth]{figs/propmuLFR}
%     \caption{original LFR assignment}
%     \label{fig:distAllpropLFR}
% \end{subfigure}
%  \begin{subfigure}[b]{0.9\textwidth}
%     \includegraphics[width=\textwidth]{figs/propmuCN}
%     \caption{CN}
%     \label{fig:distAllpropCN}
% \end{subfigure}
%  \begin{subfigure}[b]{0.9\textwidth}
%     \includegraphics[width=\textwidth]{figs/propmuNE}
%     \caption{NE}
%     \label{fig:distAllpropNE}
% \end{subfigure}
%\includegraphics[width=1\linewidth]{figs/perc_rewir_all.png}
% \includegraphics[width=1\linewidth]{figs/densiLFR.png}
% \includegraphics[width=1\linewidth]{figs/densiCN.png}
% \includegraphics[width=1\linewidth]{figs/densiNE.png}
% \caption{The probability density estimation for parameters, as they change by $\mu$.  In each plot, rows are different models: CF(top), BA(middle), FF(last). Initial network is marked by blue.}%Top: original LFR assignment, Middle: CN, Bottom: NE.
% \label{fig:distAllprop}
% \end{figure*}
% 
% \begin{figure*}
% \centering
% \begin{subfigure}[b]{0.49\textwidth}
 %   \includegraphics[width=\textwidth]{figs_/prop_dist}
%     \caption{Distribution of proberties for initial networks, for one run of the \reffig{fig:propnets}.}
%     \label{fig:nets_prop_dist}
% \end{subfigure}
% \begin{subfigure}[b]{0.49\textwidth}
%     \includegraphics[width=\textwidth]{figs/prop_pdf}
%     \caption{Probability density function estimated from all runs in \reffig{fig:propnets} for properties of the initial network, before rewiring.}
%     \label{fig:nets_prob_pdf}
% \end{subfigure}
% \end{figure*}

% \includegraphics[width=.9\linewidth]{figs/prop_dist}
% \caption{}
% \label{fig:nets_prop_dist}
% 
% \begin{figure}
% \centering
% \includegraphics[width=.9\linewidth]{figs/prop_pdf}
% \caption{}
% \label{fig:nets_prob_pdf}
% \end{figure}


% 
% \begin{figure*}
% \centering
% %\includegraphics[width=1\linewidth]{figs/perc_rewir_all.png}
% \includegraphics[width=1\linewidth]{figs/CF.png}
% \includegraphics[width=1\linewidth]{figs/AB.png}
% \includegraphics[width=1\linewidth]{figs/FF.png}
% \caption{Comparing three network models in LFR.}
% \label{fig:nets}
% \end{figure*}
%   
 %\begin{figure*}
%\centering
 %\includegraphics[width=1\linewidth]{figs/perc_rewir_all.png}
% \includegraphics[width=1\linewidth]{figs/m1.png}
% \includegraphics[width=1\linewidth]{figs/m2.png}
% \includegraphics[width=1\linewidth]{figs/m3.png}
% \caption{Comparing three network models in LFR, for $\mu=0.1$,$\mu=0.2$, and $\mu=0.3$. }
 %\label{fig:nets}
 %\end{figure*}

